Majorization-Minimization Dual Stagewise Algorithm for Generalized Lasso

The generalized lasso is a natural generalization of the celebrated lasso approach to handle structural regularization problems. Many important methods and applications fall into this framework, including fused lasso, clustered lasso, and constrained lasso. To elevate its effectiveness in large-scale problems, extensive research has been conducted on the computational strategies of generalized lasso. However, to our knowledge, most studies are under the linear setup, with limited advances in non-Gaussian and non-linear models. We propose a majorization-minimization dual stagewise (MM-DUST) algorithm to efficiently trace out the full solution paths of the generalized lasso problem. The majorization technique is incorporated to handle different convex loss functions through their quadratic majorizers. Utilizing the connection between primal and dual problems and the idea of ``slow-brewing'' from stagewise learning, the minimization step is carried out in the dual space through a sequence of simple coordinate-wise updates on the dual coefficients with a small step size. Consequently, selecting an appropriate step size enables a trade-off between statistical accuracy and computational efficiency. We analyze the computational complexity of MM-DUST and establish the uniform convergence of the approximated solution paths. Extensive simulation studies and applications with regularized logistic regression and Cox model demonstrate the effectiveness of the proposed approach.

==> thm.tex <==
\clearpage

\section{Convergence analysis}

\begin{lemma}\label{lemma1}
For a box-constrained problem with convex and differentiable objective function, if we can find a point such that the 
objective function value cannot be further reduced in any direction, then this point is the optimal solution of the problem.
\end{lemma}


\begin{theorem}
If the loss function $f(\bbeta)$ is $\mu$-strongly convex and $L$-smooth, then as the step size $\varepsilon \rightarrow 0$ and when we take $N_m=1$, the MMDCD path converges to the generalized lasso path.  
\end{theorem}

Recall that in the MMDCD path algorithm, we consecutively produce the estimations of $\bbeta$ for a sequence of generalized lasso problems, in which the $t$th problem takes a fixed tuning parameter $\lambda_t$, and we have $\lambda_{t} = \lambda_{t-1} - \varepsilon$. 


Let $\hat\bbeta_t$ be the estimation of $\bbeta$ from MMDCD when the tuning parameter takes value $\lambda_t$. Consider the original optimization problem and the majorized problem at $\lambda_t$, we have
\begin{align*}
    \tilde\bbeta_t &= \arg\min \tilde g_t(\bbeta|\hat\bbeta_{t-1}) = \arg\min \tilde f(\bbeta|\hat\bbeta_{t-1}) + \lambda_t\|\D\bbeta\|_1, \\
    \bbeta_t^* &= \arg\min g_t(\bbeta) = \arg\min f(\bbeta) + \lambda_t\|\D\bbeta\|_1,
\end{align*}
where $g_t$, $f$, $\tilde g_t$, and $\tilde f$ are the objective function, loss function, majorized loss function and majorized loss function, respectively. 

By design, the $(t-1)$th estimation with tuning parameter $\lambda_{t-1}$, $\hat\bbeta_{t-1}$, is used as the initial value to construct the surrogate function in the majorization step for the $t$th optimization problem. To show that the MMDCD path converges to the generalized lasso path, we will show that
\begin{align*}
	\|\hat\bbeta_t - \bbeta_t^*\| \leq C\varepsilon, \ \forall t,
\end{align*}
where $C$ is a constant not depending on $t$ or $\varepsilon$.

The distance between the output from MMDCD, $\hat\bbeta_t$, and the exact solution $\bbeta_t^*$, can be well-bounded with 
\begin{align}\label{eq:decompose1}
    \|\hat\bbeta_t - \bbeta_t^*\| \leq \|\hat\bbeta_t - \tilde\bbeta_t\| + \|\tilde\bbeta_t - \bbeta_t^*\|.
\end{align}
We will discuss the two parts on the RHS to construct the upper bound for this distance. 

\subsection{Bound $\|\hat\bbeta_t - \tilde\bbeta_t\|$}

The first part on the RHS of \eqref{eq:decompose1} measures the distance between the optimal solution of the majorized problem and the output from MMDCD. Based on the primal-dual relationship, we have
\begin{align*}
    \tilde\bbeta_t &= \hat\bbeta_{t-1} - \frac{1}{L}(\D^{\trans}\tilde\u_t + \nabla f(\hat\bbeta_{t-1})).
\end{align*}
Each of the dual problem in MMDCD is a convex box-constraint problem with closed form. From Lemma~\ref{lemma1}, the optimal solution for the dual problem can always be obtained after sufficient iterations from the Dual-Solver. Since the dual problem may have multiple optimal points, we take $\tilde\u_t$ as the optimal point that requires the fewest dual updating steps, $N_t$. Further, we take $N_0 = \max_t N_t$.

On the other hand, from the updating rule of MMDCD, we also have
\begin{align*}
    \hat\bbeta_t &=  \hat\bbeta_{t-1} - \frac{1}{L}(\D^{\trans}\hat\u_t + \nabla f(\hat\bbeta_{t-1})),
\end{align*}
where $\hat\u_t$ is the output from MMDCD. 
As we restrict the maximum number of dual iterations as $N_d$, the result from MMDCD, $\hat\u_t$, can be different from $\tilde \u_t$. It then follows that 
\begin{align}\label{eq:part1}
    \|\hat\bbeta_t - \tilde\bbeta_t\| \leq \frac{1}{L}\|\D(\hat\u_t - \tilde\u_t)\| 
    \leq \frac{1}{L}\|\D\|_F\|\hat\u_t - \tilde\u_t\| \leq \frac{1}{L}\|\D\|_F|N_0-N_d|\sqrt{m}\varepsilon.
\end{align}
The last inequality follows from the fact that in each of the dual updates, at most $m$ elements of $\u$ are updated by the fixed step size $\varepsilon$.




%=========================================================
\subsection{Bound $\|\tilde\bbeta_t - \bbeta_t^*\|$}

The second part in \eqref{eq:decompose1} measures the distance between the optimal point of the exact objective $g_t$ and the majorized objective $\tilde g_t$. Assume that the loss function $f$ is $\mu$-strongly convex, $L$-smooth, and twice-differentiable. %We first show that the objective function $g$ is also $\mu$-strongly convex.


Based on the $\mu$-strongly convexity of $f$, for $\forall \bbeta_1$, $\bbeta_2\in\mathcal{R}^p$, we have
\begin{align*}
    f(\bbeta_1) \geq f(\bbeta_2) + \nabla f(\bbeta_2)^{\trans}(\bbeta_1 - \bbeta_2) + \frac{\mu}{2}\|\bbeta_1-\bbeta_2\|^2.
\end{align*}
Since the penalty function is also convex, we also have 
\begin{align*}
    \lambda\|\D\bbeta_1\|_1 \geq \lambda\|\D\bbeta_2\|_1 + \lambda(\D^{\trans}\bdelta_2)^{\trans}(\bbeta_1 -\bbeta_2),
\end{align*}
where $\bdelta_2\in\mathcal{R}^m$ takes value $\sgn(\D\bbeta_2)_i$ at the $i$th position. Therefore, we can get 
\begin{align}\label{eq:stronglyconvex}
    g(\bbeta_1) \geq g(\bbeta_2) + (\nabla f(\bbeta_2) + \lambda\D^{\trans}\bdelta_2)^{\trans}(\bbeta_1-\bbeta_2) + \frac{\mu}{2}\|\bbeta_1 - \bbeta_2\|^2,
\end{align}
where $\nabla f(\bbeta_2) + \lambda\D^{\trans}\bdelta_2 = \partial g(\bbeta_2)$ is the partial derivative of the objective function $g$ evaluated at $\bbeta_2$. 
%It indicates that $g$ is also $\mu$-strongly convex. 
Set $\bbeta_1=\tilde\bbeta_t$ and $\bbeta_2=\bbeta_t^*$. By definition of $\bbeta_t^*$, we have $\bzero \in \nabla f(\bbeta_t^*) + \lambda_t\D^{\trans}\bdelta_t$. It indicates that
\begin{align}\label{eq:bound1}
    g_t(\tilde\bbeta_t) \geq g_t(\bbeta_t^*) + \frac{\mu}{2}\|\bbeta_t^* - \tilde\bbeta_t\|^2.
\end{align}



Recall that in the MMDCD algorithm, we take the majorized objective function as 
\begin{align*}
    \tilde g_t(\bbeta|\hat\bbeta_{t-1}) = f(\hat\bbeta_{t-1}) + \nabla f(\hat\bbeta_{t-1})^{\trans}(\bbeta - \hat\bbeta_{t-1}) + 
    \frac{L}{2}\|\bbeta - \hat\bbeta_{t-1}\|^2 + \lambda_t\|\D\bbeta\|_1
\end{align*}
with $L$ being the Lipschitz continous constant of the loss function $f$. 
Define $h_t(\bbeta) = \tilde g_t(\bbeta|\hat\bbeta_{t-1}) - g_t(\bbeta)$. Then
\begin{align*}
    h_t(\bbeta) 
    &= f(\hat\bbeta_{t-1}) - f(\bbeta) + \nabla f(\hat\bbeta_{t-1})^{\trans}(\bbeta - \hat\bbeta_{t-1}) + 
    \frac{L}{2}\|\bbeta - \hat\bbeta_{t-1}\|^2, \\
    \nabla h_t(\bbeta) &= -\nabla f(\bbeta) + \nabla f(\hat\bbeta_{t-1}) + L(\bbeta-\hat\bbeta_{t-1}), \\
    \nabla^2 h_t(\bbeta) &= L\I - \nabla^2 f(\bbeta).
\end{align*}
Since both $L\I - \nabla^2 f(\bbeta)$ and $L\I -(L\I - \nabla^2 f(\bbeta))$ are positive semi-definite for all $\bbeta$, the function $h_t$ is convex and $L$-smooth. Consequently, we get
\begin{align}\label{eq:bound2}
    h_t(\bbeta_t^*) &\leq h_t(\hat\bbeta_{t-1}) + \nabla h_t(\hat\bbeta_{t-1})^{\trans}(\bbeta_t^* - \hat\bbeta_{t-1}) + \frac{L}{2}\|\bbeta_t^* - \hat\bbeta_{t-1}\|^2, \notag \\
    |h_t(\bbeta_t^*)| &\leq \frac{L}{2}\|\bbeta_t^* - \hat\bbeta_{t-1}\|^2,
\end{align}
where the second inequality follows from the facts that $h_t(\hat\bbeta_{t-1})=0$ and $\nabla h_t(\hat\bbeta_{t-1})=\bzero$.


On the other hand, the second order gradient of the majorized loss function $\tilde f(\bbeta|\hat\bbeta_{t=1})$ equals to $L\I$, which indicates that the majorized loss is $L$-strongly convex. By the same arguments we used to show \eqref{eq:stronglyconvex}, it is straightforward to verify that $\tilde g_t(\bbeta|\hat\bbeta_{t-1})$ is $L$-strongly convex. Thus, we can get
\begin{align*}
    \tilde g_t(\bbeta_t^*|\hat\bbeta_{t-1}) \geq \tilde g_t(\tilde \bbeta_t|\hat\bbeta_{t-1}) + 
    \partial\tilde g_t(\tilde\bbeta_t|\hat\bbeta_{t-1})^{\trans}(\bbeta_t^* - \tilde\bbeta_t) + \frac{L}{2}\|\bbeta_t^* - \tilde\bbeta_t\|^2.
\end{align*}
As $\tilde\bbeta_t \in \arg\min \tilde g_t(\bbeta|\hat\bbeta_{t-1})$, $\bzero \in \partial\tilde g_t(\tilde\bbeta_t|\hat\bbeta_{t-1})$. As a consequence, 
\begin{align}\label{eq:bound3}
    \tilde g_t(\bbeta_t^*|\hat\bbeta_{t-1}) \geq \tilde g_t(\tilde \bbeta_t|\hat\bbeta_{t-1}) + 
     \frac{L}{2}\|\bbeta_t^* - \tilde\bbeta_t\|^2.
\end{align}

According to the property of the majorization step, we also have $g_t(\tilde\bbeta_t) \leq \tilde g_t(\tilde\bbeta_t|\hat\bbeta_{t-1})$. Combining this property with  inequalities \eqref{eq:bound1},  \eqref{eq:bound2}, and \eqref{eq:bound3}, we get
\begin{align*}
    g_t(\tilde\bbeta_t) + \frac{L}{2}\|\bbeta_t^* - \tilde\bbeta_t\|^2 
    &\leq \tilde g_t(\bbeta_t^*|\hat\bbeta_{t-1}) \\
    &= g_t(\bbeta_t^*) + h(\bbeta_t^*) \\
    &\leq g_t(\tilde\bbeta_t) - \frac{\mu}{2}\|\bbeta_t^* - \tilde\bbeta_t\|^2 + \frac{L}{2}\|\bbeta_t^* - \hat\bbeta_{t-1}\|^2.
\end{align*}
That is 
\begin{align}\label{eq:part2}
    \|\bbeta_t^* - \tilde\bbeta_t\|^2 \leq \frac{L}{L + \mu}\|\bbeta_t^* - \hat\bbeta_{t-1}\|^2.
\end{align}
Since $L/(L+\mu)$ is smaller than $1$, inequality ~\eqref{eq:part2} indicates that for the $t$th optimization problem, the resulted estimation $\hat\bbeta_t$ from the one-time Majorization-Minimization is improved when compared with the initinal estimation $\hat\bbeta_{t-1}$. 



%===========================================================
\subsection{Bound $\|\hat\bbeta_t - \bbeta_t^*\|$}

Combining \eqref{eq:decompose1}, \eqref{eq:part1} and \eqref{eq:part2}, we get 
\begin{align}
    \|\hat\bbeta_t - \bbeta_t^*\| \leq \frac{1}{L}\|\D\|_F|N_0 - N_d|\sqrt{m}\varepsilon
    + \sqrt{\frac{L}{L+\mu}}\|\bbeta_t^* - \hat\bbeta_{t-1}\|.
\end{align}
Further, we have $\|\bbeta_t^* - \hat\bbeta_{t-1}\| \leq \|\bbeta_t^* - \bbeta_{t-1}^*\| + \|\bbeta_{t-1}^* - \hat\bbeta_{t-1}\|$.

Next, we try to bound $\|\bbeta_{t}^* - \hat\bbeta_{t-1}^*\|$ by a function of the step size $\varepsilon$. Still from the $\mu$-strongly convexity of the loss function $f$, by setting $\bbeta_1 = \bbeta_t^*$ and $\bbeta_2 = \bbeta_{t-1}^*$, we have
\begin{align*}
    g_t(\bbeta_t^*) \geq g_t(\bbeta_{t-1}^*) + (\nabla f(\bbeta_{t-1}^*) + \lambda_t\D^{\trans}\bdelta_{t-1})^{\trans}(\bbeta_t^*-\bbeta_{t-1}^*) + \frac{\mu}{2}\|\bbeta_t^* - \bbeta_{t-1}^*\|^2,
\end{align*}
where the partial derivative $\bdelta_{t-1}$ is evaluated at $\bbeta_{t-1}^*$. Since $\bbeta_t^*$ is the minima, $g_t(\bbeta_t^*) \leq g_t(\bbeta_{t-1}^*)$. Consequently, we get
\begin{align*}
    0 \geq -\|\nabla f(\bbeta_{t-1}^*) + \lambda_t\D^{\trans}\bdelta_{t-1}\| \|\bbeta_t^* - \bbeta_{t-1}^*\| + \frac{\mu}{2}\|\bbeta_t^* - \bbeta_{t-1}^*\|^2.
\end{align*}

It then follows that 
\begin{align*}
    \|\bbeta_t^* - \bbeta_{t-1}^*\| 
    & \leq \frac{2}{\mu}\|\nabla f(\bbeta_{t-1}^*) + \lambda_t\D^{\trans}\bdelta_{t-1}\| \\
    & \leq \frac{2}{\mu}\|\nabla f(\bbeta_{t-1}^*) + (\lambda_t+\varepsilon)\D^{\trans}\bdelta_{t-1} - \varepsilon\D^{\trans}\bdelta_{t-1}\| \\
    & \leq \frac{2}{\mu}\|\varepsilon\D^{\trans}\bdelta_{t-1}\| \\
    & \leq \frac{2}{\mu}\varepsilon \|\D\|_F\sqrt{m}.
\end{align*}
The third inequality follows from the fact that  $\lambda_t + \varepsilon = \lambda_{t-1}$ and $\bzero \in \nabla f(\bbeta_{t-1}^*) + \lambda_{t-1}\D^{\trans}\bdelta_{t-1} = \partial g_{t-1}(\bbeta_{t-1}^*)$, as $\bbeta_{t-1}^*$ is the mimia of the optimization problem at $\lambda_{t-1}$. 

Let $c = \sqrt{L/(L + \mu)}$ and $c_0 = 1/L\|\D\|_F|N_t - N_d| \sqrt{m}\varepsilon + 
	2c/\mu\varepsilon \|\D\|_F\sqrt{m}$. Finally, we get
\begin{align*}
	\|\hat\bbeta_t - \bbeta_t^*\| 
	& \leq \frac{1}{L}\|\D\|_F|N_0- N_d| \sqrt{m}\varepsilon + 
	c\|\bbeta_t^* - \bbeta_{t-1}^*\| \\
	& \leq \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0 - N_d|  + 
	\frac{2c}{\mu}) +
	c \|\hat\bbeta_{t-1} - \bbeta_{t-1}^*\| \\
	%& = \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_t - N_d|  + 
	%\frac{2c}{\mu} + c\|\hat\bbeta_{t-1} - \bbeta_{t-1}^*\| \\
	& \leq \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0 - N_d|  + 
	\frac{2c}{\mu}) + c\left( \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0 - N_d|  + 
	\frac{2c}{\mu}) + c\|\hat\bbeta_{t-2} - \bbeta_{t-2}^*\|\right) \\
	& \leq \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0 - N_d|  + 
	\frac{2c}{\mu})(1 + c + c^2 + \ldots, + c^{t-2}) + c^{t-1}\|\hat\bbeta_1 - \bbeta_1^*\| \\
    & \leq \varepsilon\sqrt{m}\|\D\|_F\frac{1}{L}|N_0 - N_d|(1 + c + c^2 + \ldots, + c^{t-1}) \\
    & + \varepsilon\sqrt{m}\|\D\|_F\frac{2c}{\mu}(1 + c + c^2 + \ldots, + c^{t-2}) 
    + c^t\|\bbeta_1^* - \hat\bbeta_0\| \\
	& \leq \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0 - N_d|  +
	\frac{2c}{\mu}) 
	\frac{1-c^t}{1-c} + c^t\|\hat\bbeta_0 - \bbeta_0^*\| \\
	& \leq \frac{1}{1-c} \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0- N_d|  + 
	\frac{2c}{\mu})+ c^t\|\hat\bbeta_0 - \bbeta_0^*\|.
\end{align*}


By design of Algorithm~\ref{alg:mmdcd}, $\bbeta_0^*$
By design, when the original loss function is strongly convex, the first optimization problem %with tuning parameter $\lambda_{max}$ 
can be fully solved. Thus, $\|\hat\bbeta_0 - \bbeta_0^*\|=0$. %Further, we have $t = \lambda_{max}/\varepsilon$. 
Since $c<1$, it follows that $\|\hat\bbeta_t - \bbeta_t^*\|  \rightarrow 0$ as $\varepsilon \rightarrow 0$.
%as long as
%\begin{align*}
%	\frac{1}{1-c} \varepsilon\sqrt{m}\|\D\|_F(\frac{1}{L}|N_0- N_d|  + 
%	\frac{2c}{\mu}) = \mathcal{O}(\varepsilon).
%\end{align*}





This completes the proof. 
 




==> thm_backup.tex <==
Without loss of generality, we rewrite the box-constrained problem ~\eqref{eq:dual} as 
\begin{align}
    \mathop{\mbox{minimize}}\limits_{\u}\ f(\u), \mbox{ s.t. } \|\u\|_{\infty} \leq \lambda,
\end{align}
where $f$ is a convex and differentiable function and $\u\in\mathbb{R}^m$. The original constraint can be formulated as $I(\|\u\|_{\infty} \leq\lambda)=0$, which can be further decomposed into $m$ coordinate-wise constraints $h_i(\u) = I(-\lambda \leq u_i \leq \lambda)=0$, for $i=1, 2, \ldots, m$. Here, the indicator function $I(\cdot)$ equals to 0 when the conditions are satisfied and infinity otherwise. 
It follows that an equivalent Lagrangian form 
of the box-constrained problem can be formulated as
\begin{align}
    \mathop{\mbox{minimize}}\limits_{\u}\ f(\u) + \sum_{i=1}^m s_ih_i(\u),
    \label{eq:box-constrained}
\end{align}
where $s_i, \ i=1, 2, \ldots, m$ are a positive scalars. 
It is obvious that the objective function in problem~\eqref{eq:box-constrained} has a convex and differentiable part $f(\u)$, and a convex, separable but non-smooth part $\sum_{i=1}^m s_ih_i(\u)$. Consequently, optimization of \eqref{eq:box-constrained} in each direction of $\u$ is a convex problem. 

Assume that we have found a point $\u_0$, such that the objective function $f(\u)$ cannot be further reduced in any feasible directions of $\u$. It indicates that for each direction $i$, we have
\begin{align*}
    0 \in \nabla_i f(\u_0) + s_i\partial h_i(\u_0) \Leftrightarrow -\nabla_i f(\u_0) \in s_i\partial h_i(\u_0),
\end{align*}
where $\partial h_i(\u)$ is the subgradient of $h_i$.
%Moreover, to maintain feasibility, we also have $h_i(\u)=0$ for all $i$. 
According to the definition of subgradient, for $\forall \u\in\mathbb{R}^m$, we further have
\begin{align*}
    h_i(\u) \geq h_i(\u_0) + \partial h_i(\u)(u_i-u_{0i})\ \Rightarrow\  s_ih_i(\u) \geq s_ih_i(\u_0) - \nabla_i f(\u_0)(u_i-u_{0i}).
\end{align*}



Hence, based on the first order inequality of the convex function, 
\begin{align*}
    f(\u) + \sum_{i=1}^m s_ih_i(\u) - (f(\u_0) + \sum_{i=1}^m s_ih_i(\u_0)) &\geq \nabla f(\u_0)^{\trans}(\u-\u_0) + \sum_{i=1}^m s_i[h_i(\u)-h_i(\u_0)] \\
    & = \sum_{i=1}^m \nabla_i f(\u_0)(u_i-u_{0i})+ \sum_{i=1}^m s_i[h_i(\u)-h_i(\u_0)] \\
    & \geq 0.
\end{align*}
It indicates that $f(\u_0)$ is the minimum of $f(\u)$ under the box-constraints. This completes the proof.


\begin{lemma}\label{lemma1}
For a box-constrained problem with convex and differentiable objective function, if we can find a point such that the 
objective function value cannot be further reduced in any feasible direction, then this point is the optimal solution of the problem.
\end{lemma}
